Analyzing FreeRTOS Scheduling Behaviors with the Spin Model Checker

FreeRTOS is a real-time operating system with configurable scheduling policies. Its portability and configurability make FreeRTOS one of the most popular real-time operating systems for embedded devices. We formally analyze the FreeRTOS scheduler on ARM Cortex-M4 processor in this work. Specifically, we build a formal model for the FreeRTOS ARM Cortex-M4 port and apply model checking to find errors in our models for FreeRTOS example applications. Intriguingly, several errors are found in our application models under different scheduling policies. In order to confirm our findings, we modify application programs distributed by FreeRTOS and reproduce assertion failures on the STM32F429I-DISC1 board.

==> S_FreeRTOS.tex <==

\section{Execution Units}

Our goal is to develop \promela models for example applications, the
FreeRTOS scheduler with its task synchronization functions, and the
ARM Cortex-M4 interrupt mechanism. An application has a number of
tasks to be executed by the processor. When an interrupt is triggered,
its interrupt handler will be executed by the processor. We therefore
say a task or an interrupt handler are \emph{execution units}.
In our \promela model, an execution unit is formalized as a \promela
process. Commands in the \promela process thus specify the computation
of the execution unit. 

\hide{
FreeRTOS is designed to run on a single processing core. Consequently,
only a task or an interrupt handler can be executed by the processor
at any time. We hence call a task or an interrupt handler an
\emph{execution unit}. When an execution unit starts running, it
continues doing so until it is preempted by FreeRTOS scheduler or
another interrupt handler.
}

\hide{
\begin{figure}
\begin{lstlisting}[language=PROMELA,mathescape=true]
#define AWAIT(id, cmd) atomic { EP==id -> cmd }
#define SELE(id, bexp) ( EP==id && (bexp) )
#define ELSE(id, bexp) ( EP==id && !(bexp) )
proctype ExecUnit() {
  AWAIT($\mathit{id}$, $\mathit{cmd}_0$); AWAIT($\mathit{id}$, $\mathit{cmd}_1$);
  if
  :: SELE($\mathit{id}$, $\mathit{bexp}_{2}$) -> AWAIT($\mathit{id}$, $\mathit{cmd}_{20}$);
  :: ELSE($\mathit{id}$, $\mathit{bexp}_{3}$)
  fi; }
\end{lstlisting}
\caption{Execution Unit Model}
\label{fig:seq}
\end{figure}

Figure~\ref{fig:seq} 
The macro
\texttt{AWAIT(}$\mathit{id}$\texttt{,}$\mathit{cmd}$\texttt{)} expands
to \texttt{atomic \{ EP == } $\mathit{id}$ \texttt{ -> }
$\mathit{cmd}$ \texttt{ \}}. Effectively, $\mathit{cmd}$ is enabled
when the condition \texttt{ EP == } $\mathit{id}$ holds. For each
command $\mathit{cmd}$ in the execution unit with the identification
number $\mathit{id}$, \texttt{AWAIT(}$\mathit{id}$\texttt{,}
$\mathit{cmd}$\texttt{)} ensures $\mathit{cmd}$ is executed only when
the global variable \texttt{EP} is equal to the identification number
$\mathit{id}$ of the execution unit.
Similarly, \texttt{SELE(}$\mathit{id}$\texttt{,}$\mathit{bexp}$\texttt{)}
and \texttt{ELSE(}$\mathit{id}$\texttt{,}$\mathit{bexp}$\texttt{)} add the
condition \texttt{EP == }$\mathit{id}$ in conjunction with the Boolean
expression $\mathit{bexp}$ and its negation respectively. They ensure
the Boolean expression $\mathit{bexp}$ or its negation is only checked
when the global variable \texttt{EP} is equal to the identification number
$\mathit{id}$. Using these macros, it is easy to model continuous
execution in an execution unit. It suffices to use \texttt{AWAIT} for each
command, and \texttt{SELE} or \texttt{ELSE} for each Boolean expression
with the identification number of the execution unit. The global
variable \texttt{EP} determines which execution unit is running
without interleavings.
}

\subsection{Task}

Typical FreeRTOS tasks loop forever and never terminate. Their models
are \promela processes with infinite loops (Fig.~\ref{fig:task}).
In \promela, an enabled command is executed non-deterministically
among all such commands in all processes. Our FreeRTOS task models
however need be scheduled by our formal scheduler model before
execution. To this end, we define the global variable
\texttt{EP} (for Executing Process) and assign each execution unit a
unique identification number. Every guards and commands in task models
are annotated with the condition \texttt{EP} \texttt{==}
$\mathit{id}$. The FreeRTOS scheduler model in turn assigns the
variable \texttt{EP} to decide which task model is to be executed.

More precisely, each guard $\mathit{bexp}$ is annotated
with the macros 
\texttt{SELE(}$\mathit{id}$\texttt{,}$\mathit{bexp}$\texttt{)} or
\texttt{ELSE(}$\mathit{id}$\texttt{,}$\mathit{bexp}$\texttt{)};
each command $\mathit{cmd}$ is annotated with
\texttt{AWAIT(}$\mathit{id}$\texttt{,}$\mathit{cmd}$\texttt{)}.
The macros \texttt{SELE(}$\mathit{id}$\texttt{,}$\mathit{bexp}$\texttt{)}
and \texttt{ELSE(}$\mathit{id}$\texttt{,}$\mathit{bexp}$\texttt{)} add the
condition \texttt{EP} \texttt{==} $\mathit{id}$ in conjunction with the Boolean
expression $\mathit{bexp}$ and its negation respectively. If the task
model is not scheduled for execution, the variable \texttt{EP} is not
equal to its identification number and the annotated guard is
false. Otherwise, the variable \texttt{EP} is set to its
identification number and the guard $\mathit{bexp}$ is then
checked. The macro
\texttt{AWAIT(}$\mathit{id}$\texttt{,}$\mathit{cmd}$\texttt{)} expands 
on the other hand annotates the guard \texttt{EP} \texttt{==} $\mathit{id}$
to the command $\mathit{cmd}$. The annotated command is enabled
precisely when the task model is scheduled for execution.

\begin{figure}
\begin{lstlisting}[language=PROMELA,mathescape=true]
#define SELE($\mathit{id}$, $\mathit{bexp}$) ( EP==$\mathit{id}$ && ($\mathit{bexp}$) )
#define ELSE($\mathit{id}$, $\mathit{bexp}$) ( EP==$\mathit{id}$ && !($\mathit{bexp}$) )
#define AWAIT($\mathit{id}$, $\mathit{cmd}$) atomic { EP==$\mathit{id}$ -> $\mathit{cmd}$ }
proctype task() {
do
:: SELE($\mathit{id}$, $\mathit{bexp}_0$) -> AWAIT($\mathit{id}$, $\mathit{cmd}_{00}$); ... AWAIT($\mathit{id}$, $\mathit{cmd}_{0n_0}$);
:: SELE($\mathit{id}$, $\mathit{bexp}_1$) -> AWAIT($\mathit{id}$, $\mathit{cmd}_{10}$); ... AWAIT($\mathit{id}$, $\mathit{cmd}_{1n_1}$);
:: ...
:: SELE($\mathit{id}$, $\mathit{bexp}_k$) -> AWAIT($\mathit{id}$, $\mathit{cmd}_{k0}$); ... AWAIT($\mathit{id}$, $\mathit{cmd}_{kn_k}$);
od }
\end{lstlisting}
\caption{A Task Model}
\label{fig:task}
\end{figure}

\subsection{ARM Cortex-M4 Interrupt Handler}

For ARM Cortex-M4 processors, an interrupt is triggered when it is set to
\emph{pending} state. When an interrupt is pending, the processor decides
whether the current execution should be interrupted. If the pending
interrupt has a priority over the current execution and is unmasked,
the current execution is interrupted to execute the interrupt handler of
the pending interrupt. 

Bookkeeping is needed when the current execution is interrupted.
At \emph{exception entry}, the current processor state is pushed onto
a stack, the pending state of the interrupt is clear, and the
processor is prepared to execute the interrupt handler. The interrupt
handler is then executed during the \emph{exception taken} phase. When
the interrupt handler finishes its execution, the interrupted
processor state is restored at \emph{exception return}. The
interrupted execution is then resumed.

Recall that a triggered interrupt remains pending when it does not
have a priority over the current execution or is masked. At exception
return, the processor checks if there is any pending interrupt with a
priority over the topmost processor state on the stack. If so,
exception return is bypassed and the pending interrupt moves to
exception entry. This optimization is called \emph{tail chaining}.
In FreeRTOS, interrupts are masked or unmasked by tasks. After
interrupts are masked or unmasked, tasks invoke memory barrier
instructions to notify the processor about mask
changes~\cite{Note321}. The processor then decides if any pending
interrupt should move to exception entry.

\hide{
A distinct feature of our formalization is to give a detailed model
for ARMv7-M interrupts. Indeed, interrupts are crucial in
implementing FreeRTOS scheduling policies. Interrupt handling
mechanisms moreover vary between architectures. In order to analyze
FreeRTOS correctly, it is important to model interrupts carefully in
our formalization. In this subsection, we briefly describe the
interrupt handling mechanism in the ARMv7-M architecture and
illustrate how it is modeled in \promela.
}

Figure~\ref{fig:isr} gives the outline of an interrupt handler model.
Inside an interrupt handler model with the identificatin number $id$
is an infinite loop containing a sequence of commands. The macro
\texttt{IRQ($id$, PENDING$_\mathit{id}$)}
(for interrupt request) checks the interrupt conditions before
exception entry. In the macro, the Boolean variables
\texttt{PENDING}$_{id}$ and \texttt{MASKED}$_{id}$ denote whether the
interrupt $id$ is pending or masked respectively.
\texttt{PRIORITIZING(}$id$\texttt{, EP)} checks if the interrupt has
the priority over the current running execution unit. 
\texttt{IRQ($id$, PENDING$_\mathit{id}$)} executes another macro
\texttt{ExpEntry(}$id$\texttt{)} if all conditions are satisified.
In \texttt{ExpEntry(}$id$\texttt{)}, the current execution unit
identification number is pushed on a stack, \texttt{PENDING}$_{id}$ is
set to \texttt{false}, and the variable \texttt{EP} is assigned to the
identification number $id$ of the interrupt handler model. Commmands
in the interrupt handler model can then executed.
After the interrupt handler model finishes, the \texttt{ExpReturn()}
macro is used to pop an identification number from the stack and
assigns it to the variable \texttt{EP}. The interrupted execution unit
can then continue.

\hide{ % amendment

When an interrupt is triggered, the processor first checks whether the
interrupt is unmasked and has priority over the current execution. If
so, the corresponding interrupt handler is executed and the current
execution is postponed. Otherwise, the interrupt is set to the
\emph{pending} state. A pending interrupt must wait until it is
unmasked and has sufficient priorities before its interrupt handler is
executed.

Bookkeeping tasks need to be performed when the processor decides to
interrupt the current execution.
Since the interrupted execution will be resumed later, it is
essential to save the processor state before and restore the processor
state after executing the interrupt handler.
For the ARMv7-M architecture, interrupts are
handled in three phrases. At \emph{exception entry}, the interrupted
processor state is pushed to a stack. The \emph{exception taken} phase
executes the interrupt handler. After the interrupt handler finishes
its execution, the interrupted processor state is restored from the
stack at \emph{exception return}. The processor then resumes the
interrupted execution.

Figure~\ref{fig:isr} gives the outline of an interrupt handler as a
\promela process. Inside an interrupt handler model is an infinite
loop containing a sequence of commands. The parameter $id$ is the
identification number assigned to the execution unit.
The macro \texttt{IRQ($id$, $\mathit{TRIG}$)} (for interrupt request)
models the
exception entry and taken phases. In the macro, $\mathit{TRIG}$
specifies the condition when the interrupt is triggered. If the triggered
interrupt is not pending, \texttt{IRQ($id$, $\mathit{TRIG}$)} pushes
the current
\texttt{EP} on the stack and execute the interrupt handler with the
identification number $id$. If the interrupt is pending, the
\texttt{IRQ($id$, $\mathit{TRIG}$)} macro waits until \texttt{EP} is
equal to $id$ and
then starts the exception taken phase. After
\texttt{IRQ($id$, $\mathit{TRIG}$)}, the
interrupt handler executes its commands. Finally, the
\texttt{ExpReturn()} macro checks the condition for tail-chaining. If
the pending interrupt (\texttt{PENDING\_INT()}) has a higher priority
than the execution unit on the top of the stack (\texttt{PEEK()}), the
variable \texttt{EP} is set to the identification number of the
pending interrupt handler. Otherwise, \texttt{EP} is assigned to the
execution unit on the stack (\texttt{POP()}).

} % end amendment

\begin{figure}
\begin{lstlisting}[language=PROMELA,mathescape=true]
#define ExpEntry($id$) PUSH(EP); PENDING$_{id}$=false; EP=$id$
#define ExpReturn() $\,\,$EP=POP()
#define IRQ($id$, PENDING$_\mathit{id}$)                              $\,\,$\
  if                                                $\,\,$\
  :: PENDING$_\mathit{id}$ && !MASKED$_\mathit{id}$ && PRIORITIZING($id$, EP) -> \
     ExpEntry($id$);                                    $\,\,$\
  fi
proctype interrupt_handler() {
  do
  :: atomic { IRQ($id$, PENDING$_\mathit{id}$) };
     AWAIT($id$, $\mathit{cmd}_0$); AWAIT($id$, $\mathit{cmd}_1$); ...
     AWAIT($id$, ExpReturn());
  od }
\end{lstlisting}
\caption{An Interrupt Handler Model}
\label{fig:isr}
\end{figure}

When an interrupt is pending but masked, \texttt{MASK}$_\mathit{id}$
is \texttt{true} in our model. The interrupt handler model will not
execute \texttt{ExpEntry(}$\mathit{id}$\texttt{)}. Instead, the
interrupt waits until \texttt{MASK}$_\mathit{id}$ becomes
\texttt{false}. Whenever an execution unit assigns
\texttt{MASK}$_\mathit{id}$ to \texttt{false}, it also sets
\texttt{EP} to $\mathit{id}$. The pending interrupt can check if it
should execute \texttt{ExpEntry(}$\mathit{id}$\texttt{)}.

Finally, an interrupt may remain pending when it does not have the
priority over the running execution unit
(\texttt{PRIORITIZING(}$\mathit{id}$\texttt{, EP)} is
\texttt{false}). When the interrupt with the priority finishes, the
interrupt handler will be taken without exception entry by tailing
chaining. Our interrupt handler model also performs tail chaining when
an interrupt is pending due to insufficient priorities (not shown in
Figure~\ref{fig:isr}).

\hide { % amendment

In order to improve performance, the ARMv7-M architecture further
optimize the interrupt handling mechanism by \emph{tail-chaining}.
Consider an interrupt is pending while an interrupt handler is running
by the processor. When the interrupt handler finishes, the processor
will restore the interrupted processor state from the stack in the
Exception return phase and resume the interrupted execution.
If the pending interrupt has the priority, the resumed execution
will be interrupted immediately. The processor will save the processor
state on the stack and execute the handler of the pending interrupt.
Note that the processor state is unnecessarily restored and saved on the
stack. Tail-chaining is developed to avoid such redundancy.
At the Exception return phase, the processor checks whether there is
any pending interrupt with priorities over the topmost execution on
the stack. If so, exception return is bypassed and the handler of the
pending interrupt enters the exception taken phase immediately by tail
chaining. The topmost processor state remains intact as if it is
restored and then saved on the stack. Redundant exception phases
are removed.

} % end amendment

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{FreeRTOS Scheduler}

The FreeRTOS scheduler implements three scheduling policies. 
In \emph{cooperative scheduling}, a running task has to yield the
processor explicitly by itself. In \emph{preemptive scheduling without
  time slicing}, a running task can be preempted by tasks with higher
priorities. Finally, a task can moreover be preempted by using up its
time slice in \emph{preemptive scheduling with time slicing}.
Depending on the policy, the FreeRTOS scheduler is called to elect the
next task for execution at different occasions.

In the FreeRTOS ARM Cortex-M4 port, scheduling policies are
implemented via two interrupt handlers. The interrupt handler for the
software interrupt \emph{PendSV} is used for task scheduling and
context switching. More precisely, the PendSV interrupt handler calls
the FreeRTOS scheduler to elect the next task for execution. After a
task is elected, the scheduler sets up the processor state by the
ARM Cortex-M4 interrupt handling mechanism for context switching. 
After exception return, the context of the newly elected task is
restored. The elected task resumes its computation as if it were just
returned from an interrupt handler. The PendSV interrupt is therefore
triggered whenever a task needs to be elected in all scheduling
policies.

For preemptive scheduling with time slicing, the PendSV interrupt
needs to be triggered at every time slice periodically. This is
implemented with the \emph{SysTick} interrupt. The SysTick interrupt
is triggered by a hardware clock periodically. If preemptive
scheduling is required, the SysTick interrupt handler triggers the
PendSV interrupt. When the SysTick interrupt handler finishes, the
PendSV interrupt handler will be executed directly through tail chaining.

% \subsubsection{The Scheduler Model}

\begin{figure}
  \begin{lstlisting}[language=PROMELA,mathescape=true]
proctype PendSV_handler() {
  do
  :: atomic { IRQ(PID$_\mathtt{PendSV}$, PENDING$_\mathtt{PendSV}$) } ->
       AWAIT(PID$_\mathtt{PendSV}$, SET_TOP(NextTaskId()));
       AWAIT(PID$_\mathtt{PendSV}$, ExpReturn());
  od }
proctype SysTick_handler() {
  do
  :: atomic { IRQ(PID$_\mathtt{SysTick}$, PENDING$_\mathtt{SysTick}$) } ->
       /* Process delayed/suspended tasks */
#ifdef PREEMPTIVE_SCHEDULING
       AWAIT(PID$_\mathtt{SysTick}$, PENDING$_\mathtt{PendSV}$ = true);
#endif
       AWAIT(PID$_\mathtt{SysTick}$, ExpReturn());
  od }
\end{lstlisting}
\caption{PendSV and SysTick Interrupt Handler Models}
\label{fig:pendsv-systick}
\end{figure}

Our \promela model follows the FreeRTOS ARM Cortex-M4 port to specify
the scheduler in interrupt handler models for PendSV and SysTick
(Figure~\ref{fig:pendsv-systick}). Both interrupt handler models use
\texttt{IRQ(PID$_\mathit{id}$, PENDING$_\mathit{id}$)} for interrupt
requests and exception entry. When the PendSV interrupt handler
model is taken, a task identification number is chosen by
\texttt{NextTaskId()}. The chosen identification number then
replaces the identification number on the top of stack. In
\texttt{ExpReturn()}, the variable \texttt{EP} is set to the chosen
identification number on stack. The elected task model can continue
its commands as in the FreeRTOS ARM Cortex-M4 port.

The SysTick interrupt handler model is similar
(Figure~\ref{fig:pendsv-systick}). When the interrupt handler model is
taken and preemptive schedling is enabled, it triggers the PendSV
interrupt by setting \texttt{PENDING}$_\mathtt{PendSV}$ to
\texttt{true}. Presently, the PendSV interrupt has not the priority
and will keep pending. The SysTick interrupt handler model then 
executes \texttt{ExpReturn()}. The PendSV interrupt handler model will
be taken directly by tail chaining in our interrupt handler models. 
A task identification number can then be chosen by the PendSV
interrupt handler model as in real hardware.

In our model, the SysTick interrupt is triggered by setting the
variable \texttt{PENDING}$_\mathtt{SysTick}$ to \texttt{true}. 
Since the \promela language is timeless, our model cannot assign
\texttt{PENDING}$_\mathtt{SysTick}$ periodically. Rather, our model
non-deterministically set the variable to \texttt{true}. 
Effectively, the SysTick interrupt is triggered arbitrarily in our
formalization. This is a simple but useful abstraction in our model.
% In reality, every tasks perform different functions and hence have
% different execution time. It is extremely difficult (if not
% impossible) to model SysTick interrupts accurately.
The conservative abstraction ensures that all SysTick interrupt
sequences in real world are subsumed in our model. If there is any
failure among all real interrupt sequences, it will be exposed in our
model. On the other hand, not all interrupt sequences in our model are
realistic. An error found in the model can be spurious. It has to be
validated by corresponding failures in real hardware.

\hide{
After the exception entry phase in
\texttt{IRQ(PID\_SYSTICK, PENDING$_\mathit{Systick}$)}, the SysTick
interrupt handler model activates all delayed tasks with
expired delay durations. It then triggers the PendSV interrupt
(\texttt{PENDING$_\mathit{PendSV}$}) if the time slicing policy is specified
(\texttt{TIME\_SLICING}). The interrupt handler model then enters the
exception return phase. Note that the PendSV interrupt is pending when
preemptive scheduling is enabled. The SysTick exception return phase
will be optimized by tail chaining on ARM Cortex-M4 cores. Our formal
model accurately simulates tail chaining as in hardware.

For effective model checking, our formal model for FreeRTOS on the ARM
Cortex-M4 core necessarily contains simplification.
We summarize the differences between our abstract model and the real
system as follows.
\begin{enumerate}
\item \textit{Lists are bounded with atomic operations.}
  Dynamically allocated linked lists are modeled by bounded arrays
  with atomic operations to reduce the search space.
%  Bounded arrays greatly reduces the state
%  space. Atomic list operations also simplify interleavings in the
%  model. 
\item \textit{Counters are not wrapped around.}
  Counters are reset when they are not used to prevent variable
  overflow warning in \spin. In reality, counters are never reset.
\item \textit{The SysTick interrupt is triggered arbitrarily.}
  As mentioned, our formal model is timeless and triggers the SysTick
  interrupt non-deterministically. The model will have more SysTick
  interrupts than reality. 
\item \textit{The unit of task delaying is steps rather than time.}
  In our model, a task is delayed when its delay counter is set to
  a positive integer. Note that the integer is bounded to the data size
  of the delay counter. Since the delayed task
  is \bred{inactive}, it will be scheduled after it becomes active.
  It is the SysTick interrupt handler model that activates the delayed tasks.
  Every time the SysTick interrupt handler is executing, it decreases
  all the positive delay counters by one and then activates
  the delayed tasks with the zero delay.
\end{enumerate}
}

In order
to explain interaction among different execution units, we describe
two simple scheduling scenarios in our model as illustration. Note
that all scheduling policies are in fact supported in our model.

\subsection{Cooperative Scheduling without Time Slicing}

Cooperative scheduling without time slicing is perhaps the simplest
policy provided in FreeRTOS. Under the policy, the running task must
explicitly yield so that the scheduler can choose the next running
task. In our formal model, the variable \texttt{PENDING$_{PendSV}$} is
not set in the SysTick interrupt handler model to perform scheduling
(Figure~\ref{fig:pendsv-systick}). Rather, the scheduler is invoked by
the yield system call modeled as follows. 
\[
\texttt{\#define Yield($id$) AWAIT($id$, PENDING$_{PendSV}$ = 1;)}
\]
Let $id$ be the identification number of the running
task. \texttt{Yield($id$)} simply sets the PendSV
interrupt to the pending state. For simplicity, let us further
assume other interrupts are not triggered. After the variable
\texttt{PENDING$_{PendSV}$} is set, the PendSV interrupt handler
model becomes enabled (Figure~\ref{fig:pendsv-systick}). The 
identification number of the next running task will be chosen and
replace the identification number of the yielding task on stack. The
\texttt{ExpReturn()} macro will set the variable \texttt{EP} to the
identification number of the new task (Figure~\ref{fig:isr}). Our
model can proceed the execution of the selected task.

\subsection{Preemptive Scheduling without Time Slicing}

In preemptive scheduling without time slicing, the SysTick interrupt
handler checks if delayed tasks have expired delayed duration. If so,
the interrupt hander activates such delayed tasks and triggers the
PendSV interrupt for scheduling. In our formal model, the SysTick
interrupt handler model activates any delayed tasks with expired
duration (Figure~\ref{fig:pendsv-systick}). It then sets the variable
\texttt{PENDING$_{PendSV}$}. The PendSV interrupt handler model thus
becomes enabled. The identification number of the next running task
will be chosen and put on the stack for preemptive scheduling. The
variable \texttt{EP} is hence set to the identification number of the
new task by the macro \texttt{ExpReturn()} (Figure~\ref{fig:isr}). The
chosen task can proceed with its execution.

